Distributed randomized Kaczmarz for the adversarial workers

Developing large-scale distributed methods that are robust to the presence of adversarial or corrupted workers is an important part of making such methods practical for real-world problems. Here, we propose an iterative approach that is adversary-tolerant for least-squares problems. The algorithm utilizes simple statistics to guarantee convergence and is capable of learning the adversarial distributions. Additionally, the efficiency of the proposed method is shown in simulations in the presence of adversaries. The results demonstrate the great capability of such methods to tolerate different levels of adversary rates and to identify the erroneous workers with high accuracy.

==> bmacros.tex <==
%% Version: 2013-11-26
%% common packages
\usefonttheme[onlymath]{serif} % use serif for math fonts
\usepackage{hyperref}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{subfig}
\usepackage{color}
\usepackage[dvipsnames]{xcolor}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{wasysym}
\usepackage{lmodern} % to avoid font size not available warning
\usepackage{textcomp} % to avoid font warning for textbullet used in \item
\usepackage{wasysym} % useful symbols
\usepackage{dashbox} % for use of dashd box \dbox{...}
\usepackage{mathtools} % for \DeclarePairedDelimiter below
\mathtoolsset{showonlyrefs}
\usepackage{tabto}  % for \NumTabs{3} and \tab commands
%\usepackage{mathabx} % for \vvvert matrix norm
%\usepackage[ruled,vlined]{algorithm2e}


%% to reduce footnote font size
\usepackage{etoolbox}
\makeatletter
\patchcmd{\@makefntext}{\insertfootnotetext{#1}}{\insertfootnotetext{\scriptsize#1}}{}{}
\makeatother

%% begin and end backup slides
\newcommand{\backupbegin}{
   \newcounter{framenumberappendix}
   \setcounter{framenumberappendix}{\value{framenumber}}
}
\newcommand{\backupend}{
   \addtocounter{framenumberappendix}{-\value{framenumber}}
   \addtocounter{framenumber}{\value{framenumberappendix}}
}

%% one-page section title and subsection title, which skip and hide page numbers
\newcommand{\sectiononepage}[1]{
  \section{#1}
  \begin{frame}[plain,noframenumbering]\begin{center}\begin{Large}\textbf{#1}\end{Large}\end{center}\end{frame}
}
\newcommand{\subsectiononepage}[1]{
  \subsection{#1}
  \begin{frame}[plain,noframenumbering]\begin{center}\begin{Large}\textbf{#1}\end{Large}\end{center}\end{frame}
}

%% macros for commenting
\usepackage[normalem]{ulem} % to use \sout
\newcommand{\remove}[1]{{\color{Gray}\sout{#1}}}
\newcommand{\revise}[1]{{\color{blue}#1}}
\newcommand{\commwy}[1]{{\color{red}(wy: #1)}} % Wotao Yin
\newcommand{\cut}[1]{{}}

%% check and cross marks
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

%% template for beamer
\makeatletter
  \@ifclassloaded{article} % check if article is used as the documentclass
    {}% true code
    {
      %% to allow citation as footnote
      \usepackage{natbib}
      \newcommand{\citesmall}[2][]
      {
         \ifthenelse{\equal{#1}{}}
         {\begin{small}\citep{#2}\end{small}}
         {\begin{small}\citep[#1]{#2}\end{small}}
      }
      \newcommand{\citefootnote}[2][]
      {
        \footnote{
          \ifthenelse{\equal{#1}{}}
          {\begin{small}\citep{#2}\end{small}}
          {\begin{small}\citep[#1]{#2}\end{small}}
        }
      }

      %% beamer modifier
      \mode<presentation>
      {
        % page number
        %\setbeamertemplate{footline}{\insertframenumber/\inserttotalframenumber}
        \setbeamertemplate{footline}[frame number]

        % background and theme
        \setbeamertemplate{background canvas}[vertical shading][bottom=white!10,top=white!10]
        \usetheme{default}

        % section in table of contents has numbers
        \setbeamertemplate{sections/subsections in toc}[sections numbered]

        % no navigation bottoms
        \setbeamertemplate{navigation symbols}{}

        % itemize, black bullet, %150 spacing between items using "witemize"
        \setbeamertemplate{itemize items}[circle]
        \setbeamercolor{itemize item}{fg=black}
        \setbeamercolor{enumerate item}{fg=black}
        \setbeamercolor{itemize subitem}{fg=black}
        \setbeamercolor{enumerate subitem}{fg=black}
        \newenvironment{witemize}{\itemize\addtolength{\itemsep}{0.4\baselineskip}}{\enditemize}

        % itemize enumerate use normal sized texts
        \setbeamertemplate{itemize/enumerate body begin}{\normalsize}
        \setbeamertemplate{itemize/enumerate subbody begin}{\normalsize}
        \setbeamertemplate{itemize/enumerate subsubbody begin}{\normalsize}

        % block, black over gray with no shadow
        \setbeamertemplate{blocks}[rounded][shadow=false]
        \setbeamercolor{block title}{fg=black,bg=gray!40}
        \setbeamercolor{block body}{fg=black,bg=gray!10}

        % frametitle, bold, black, centered
        \setbeamertemplate{frametitle}[default][center]
        \setbeamercolor{frametitle}{fg=black}
        \setbeamerfont{frametitle}{shape=\bfseries}

        % line spacing
        \linespread{1.2}

        \setlength{\parskip}{\smallskipamount}

        % make beamer notes itemized instead of enumerated
        \AtBeginNote{%
          \let\enumerate\itemize%
          \let\endenumerate\enditemize%
        }

        % make the note page simpler
        \setbeamertemplate{note page}[compressed]
        \setbeamercolor{note page}{bg=white}
      }
    } % false code (above)
\makeatother%

%% macros for letters

\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\ve}{{\mathbf{e}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vh}{{\mathbf{h}}}
\newcommand{\vi}{{\mathbf{i}}}
\newcommand{\vj}{{\mathbf{j}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vl}{{\mathbf{l}}}
\newcommand{\vm}{{\mathbf{m}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vo}{{\mathbf{o}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vu}{{\mathbf{u}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vz}{{\mathbf{z}}}

\newcommand{\vA}{{\mathbf{A}}}
\newcommand{\vB}{{\mathbf{B}}}
\newcommand{\vC}{{\mathbf{C}}}
\newcommand{\vD}{{\mathbf{D}}}
\newcommand{\vE}{{\mathbf{E}}}
\newcommand{\vF}{{\mathbf{F}}}
\newcommand{\vG}{{\mathbf{G}}}
\newcommand{\vH}{{\mathbf{H}}}
\newcommand{\vI}{{\mathbf{I}}}
\newcommand{\vJ}{{\mathbf{J}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vL}{{\mathbf{L}}}
\newcommand{\vM}{{\mathbf{M}}}
\newcommand{\vN}{{\mathbf{N}}}
\newcommand{\vO}{{\mathbf{O}}}
\newcommand{\vP}{{\mathbf{P}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vR}{{\mathbf{R}}}
\newcommand{\vS}{{\mathbf{S}}}
\newcommand{\vT}{{\mathbf{T}}}
\newcommand{\vU}{{\mathbf{U}}}
\newcommand{\vV}{{\mathbf{V}}}
\newcommand{\vW}{{\mathbf{W}}}
\newcommand{\vX}{{\mathbf{X}}}
\newcommand{\vY}{{\mathbf{Y}}}
\newcommand{\vZ}{{\mathbf{Z}}}

\newcommand{\valpha}{{\boldsymbol \alpha}}
\newcommand{\vbeta}{{\boldsymbol \beta }}
\newcommand{\vgamma}{{\boldsymbol \gamma}}
\newcommand{\vlambda}{{\boldsymbol \lambda}}
\newcommand{\vsigma}{{\boldsymbol \sigma}}

\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}

\newcommand{\ba}{{\boldsymbol{a}}}
\newcommand{\bb}{{\boldsymbol{b}}}
\newcommand{\bc}{{\boldsymbol{c}}}
\newcommand{\bd}{{\boldsymbol{d}}}
\newcommand{\be}{{\boldsymbol{e}}}
\newcommand{\bldf}{{\boldsymbol{f}}}
\newcommand{\bg}{{\boldsymbol{g}}}
\newcommand{\bh}{{\boldsymbol{h}}}
\newcommand{\bi}{{\boldsymbol{i}}}
\newcommand{\bj}{{\boldsymbol{j}}}
\newcommand{\bk}{{\boldsymbol{k}}}
\newcommand{\bl}{{\boldsymbol{l}}}
\newcommand{\bm}{{\boldsymbol{m}}}
\newcommand{\bn}{{\boldsymbol{n}}}
\newcommand{\bo}{{\boldsymbol{o}}}
\newcommand{\bp}{{\boldsymbol{p}}}
\newcommand{\bq}{{\boldsymbol{q}}}
\newcommand{\br}{{\boldsymbol{r}}}
\newcommand{\bs}{{\boldsymbol{s}}}
\newcommand{\bt}{{\boldsymbol{t}}}
\newcommand{\bu}{{\boldsymbol{u}}}
\newcommand{\bv}{{\boldsymbol{v}}}
\newcommand{\bw}{{\boldsymbol{w}}}
\newcommand{\bx}{{\boldsymbol{x}}}
\newcommand{\by}{{\boldsymbol{y}}}
\newcommand{\bz}{{\boldsymbol{z}}}

\newcommand{\bA}{{\boldsymbol{A}}}
\newcommand{\bB}{{\boldsymbol{B}}}
\newcommand{\bC}{{\boldsymbol{C}}}
\newcommand{\bD}{{\boldsymbol{D}}}
\newcommand{\bE}{{\boldsymbol{E}}}
\newcommand{\bF}{{\boldsymbol{F}}}
\newcommand{\bG}{{\boldsymbol{G}}}
\newcommand{\bH}{{\boldsymbol{H}}}
\newcommand{\bI}{{\boldsymbol{I}}}
\newcommand{\bJ}{{\boldsymbol{J}}}
\newcommand{\bK}{{\boldsymbol{K}}}
\newcommand{\bL}{{\boldsymbol{L}}}
\newcommand{\bM}{{\boldsymbol{M}}}
\newcommand{\bN}{{\boldsymbol{N}}}
\newcommand{\bO}{{\boldsymbol{O}}}
\newcommand{\bP}{{\boldsymbol{P}}}
\newcommand{\bQ}{{\boldsymbol{Q}}}
\newcommand{\bR}{{\boldsymbol{R}}}
\newcommand{\bS}{{\boldsymbol{S}}}
\newcommand{\bT}{{\boldsymbol{T}}}
\newcommand{\bU}{{\boldsymbol{U}}}
\newcommand{\bV}{{\boldsymbol{V}}}
\newcommand{\bW}{{\boldsymbol{W}}}
\newcommand{\bX}{{\boldsymbol{X}}}
\newcommand{\bY}{{\boldsymbol{Y}}}
\newcommand{\bZ}{{\boldsymbol{Z}}}

\newcommand{\bdelta}{{\boldsymbol{\delta}}}
\newcommand{\blambda}{{\boldsymbol{\lambda}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\renewcommand{\bell}{{\boldsymbol{\ell}}}

\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\rr}{{\mathrm{r}}}

\newcommand{\rint}{{\mathrm{ri}}}

%% macros for math notions and operators

\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}
\renewcommand{\SS}{{\mathbb{S}}}
\newcommand{\SSp}{\mathbb{S}_{+}}
\newcommand{\SSpp}{\mathbb{S}_{++}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\Sign}{\mathrm{Sign}}
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\vone}{{\mathbf{1}}}
\newcommand{\Null}{{\mathrm{Null}}}
\newcommand{\dist}{{\mathrm{dist}}}
\newcommand{\Co}{{\mathbf{Co}}}

\newcommand{\op}{{\mathrm{op}}} % subscript for operator norm
\newcommand{\opt}{{\mathrm{opt}}} % subscript for optimal solution
\newcommand{\supp}{{\mathrm{supp}}} % support
\newcommand{\Prob}{{\mathrm{Prob}}} % probability
\newcommand{\Diag}{{\mathrm{Diag}}} % vector -> diagonal matrix
\newcommand{\diag}{{\mathrm{diag}}} % matrix diagonal -> vector
\newcommand{\dom}{{\mathrm{dom}}} % domain
\newcommand{\epi}{{\mathrm{epi}}} % epigraph
\newcommand{\rank}{{\mathrm{rank}}}
\newcommand{\grad}{{\nabla}}    % gradient
\newcommand{\tr}{{\mathrm{tr}}} % trace
\newcommand{\TV}{{\mathrm{TV}}} % total variation
\newcommand{\Proj}{{\mathrm{Proj}}}
\DeclareMathOperator{\shrink}{shrink} % shrinkage
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\mini}{minimize}
\DeclareMathOperator*{\maxi}{maximize}
\DeclareMathOperator*{\Min}{minimize}
\DeclareMathOperator*{\Max}{maximize}
\newcommand{\fwd}{{\mathbf{fwd}}}
\newcommand{\prox}{{\mathbf{prox}}}
\newcommand{\refl}{{\mathbf{refl}}}
\newcommand{\proj}{{\mathbf{proj}}}
\newcommand{\solve}{\stackrel{\mathrm{solve}}\longleftarrow}
\newcommand{\st}{{\quad\mathrm{s.t.}}}
\newcommand{\St}{{\quad\mathrm{subject~to}}}
\newcommand{\pt}{{\textbullet\ }}

\newcommand{\vvvert}{{\vert\kern-0.25ex\vert\kern-0.25ex\vert}}

% --- OpSplitting specific macro ---
\newcommand{\Fix}{{\mathrm{Fix}}}
\newcommand{\tnabla}{{\widetilde{\nabla}}}
\newcommand{\TFBS}{T_{\mathrm{FBS}}}
\newcommand{\TBFS}{T_{\mathrm{BFS}}}
\newcommand{\TFBFS}{T_{\mathrm{FBFS}}}
\newcommand{\TPRS}{T_{\mathrm{PRS}}}
\newcommand{\TDRS}{T_{\mathrm{DRS}}}
\newcommand{\TDYS}{T_{\mathrm{DYS}}}
\newcommand{\TPRSl}{T^\lambda_{\mathrm{PRS}}}
\newcommand{\kbest}{{k_{\mathrm{best}}}}

\DeclarePairedDelimiter{\dotp}{\langle}{\rangle}  % inner product
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}    % ceil function
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor} % floor function

%% macros for theorem-like environments

\makeatletter
  \@ifclassloaded{article} % check if article is used as the documentclass
    {
      \newtheorem{theorem}{Theorem}
      \newtheorem{definition}{Definition}
      \newtheorem{example}{Example}
    }% true code
    {} % false code
\makeatother%

\newtheorem{condition}{Condition}
\newtheorem{assumption}{Assumption}
%\newtheorem{corollary}{Corollary}
%\newtheorem{remark}{Remark}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proof}{Proof}
\newtheorem{proposition}{Proposition}

%\newtheorem{example}[remark]{Example}

